Troubling Trends in Machine Learning Scholarship

Collectively, machine learning (ML) researchers are engaged in the creation and dissemination of knowledge about data-driven algorithms. In a given paper, researchers might aspire to any subset of the following goals, among others: to theoretically characterize what is learnable, to obtain understanding through empirically rigorous experiments, or to build a working system that has high predictive accuracy. While determining which knowledge warrants inquiry may be subjective, once the topic is fixed, papers are most valuable to the community when they act in service of the reader, creating foundational knowledge and communicating as clearly as possible. Recent progress in machine learning comes despite frequent departures from these ideals. In this paper, we focus on the following four patterns that appear to us to be trending in ML scholarship: (i) failure to distinguish between explanation and speculation; (ii) failure to identify the sources of empirical gains, e.g., emphasizing unnecessary modifications to neural architectures when gains actually stem from hyper-parameter tuning; (iii) mathiness: the use of mathematics that obfuscates or impresses rather than clarifies, e.g., by confusing technical and non-technical concepts; and (iv) misuse of language, e.g., by choosing terms of art with colloquial connotations or by overloading established technical terms. While the causes behind these patterns are uncertain, possibilities include the rapid expansion of the community, the consequent thinness of the reviewer pool, and the often-misaligned incentives between scholarship and short-term measures of success (e.g., bibliometrics, attention, and entrepreneurial opportunity). While each pattern offers a corresponding remedy (don't do it), we also discuss some speculative suggestions for how the community might combat these trends.

==> sections/antecedents.tex <==
The reader may also question whether these patterns  reflect \emph{trends}
rather than the normal state of affairs.
While we perceive them to be trends,
absent a methodology to quantify them,
this may be the most subjective of our assertions.
Whether or not they are trends, 
these issues are neither unique to machine learning 
nor to this moment in time; 
they instead reflect 
issues that recur cyclically throughout academia. 
As far back as 1964, John Platt \citep{platt1964strong} discussed related concerns in his paper on strong inference, where he identified adherence to specific empirical standards as responsible for the rapid progress of molecular biology and high-energy physics relative to other areas of science.

There have also been similar discussions in AI. 
In 1976, Drew McDermott \citep{mcdermott1976artificial} chastened a (mostly pre-ML) AI community
about the dangers of abandoning self-discipline. 
He warned prophetically that ``if we can't criticize ourselves, someone else will save us the trouble'' and enumerated problems including suggestive definitions and a failure to separate out speculation from technical claims. 
In 1988, Paul Cohen and Adele Howe \cite{cohen1988evaluation} addressed an AI community 
that at that point ``rarely publish[ed] performance evaluations'' of their proposed algorithms and instead only described the systems. %Cohen and Howe go on to remark, ``we have
%faith---often  groundless  and  mislead-
%ing---that  building  programs  is  some-
%how  informative.''
They suggested establishing sensible metrics 
for quantifying progress, 
and also analyzing ``why does it work?'',
``under what circumstances won't it work?'' 
and ``have the design decisions been justified?'',
questions that continue to resonate today.
% While the current generation of ML papers 
% has improved considerably at reporting quantitative improvements, 
% we warn that these latter questions are subsequently ignored.
%
%These themes have also emerged outside 
%the immediate confines of AI/ML:
Finally, in 2009 Armstrong and co-authors \cite{armstrong2009improvements} 
discussed the empirical rigor 
of information retrieval research and 
noted a tendency of papers to compare against the same weak baselines, producing a long series of improvements that did not accumulate to meaningful gains.

In other fields, an unchecked decline in scholarship has led to crisis. A landmark study in 2015 suggested that a significant portion of findings in the psychology literature may not be reproducible \cite{open2015estimating}.
In a few historical cases, 
enthusiasm paired with undisciplined scholarship
led entire communities down blind alleys. 
For example, following the discovery of X-rays,
a related discipline on N-rays emerged \citep{nye1980n} before it was eventually debunked.
Closer to the field of machine learning, 
a whole discipline of fuzzy logic proliferated,
perhaps distracting researchers from probabilistic approaches, before a critical paper \citep{elkan1994paradoxical} pointed out some fundamental flaws in the approach.

The reader might rightly suggest that these problems are self-correcting and that ML's success are on too sure a footing to end up in crisis. However, the community self-corrects 
precisely through recurring debate about what constitutes reasonable standards for scholarship.
We hope that this paper 
contributes constructively to the discussion.

% \begin{itemize}
% \item SGD vs GD
% \item Perennial issue, not a trend.  
% \item cyclical vs trend
% \item these things happen, have happened in the past
% \item there have also been corrections in the past
% \item this paper is not outside of the process
% \item rather conversations like this are part of the mechanisms by which the field self-corrects
% \item point out all the antecedents
% \item   .
% \end{itemize}





% with words like ``thought vector'' \citep{kiros2015skip} 
% and ``consciousness prior'' \citep{bengio2017consciousness},
% when \emph{meaning} and \emph{co-occurrence} are casually interchanged, 
% and when claims of human-level performance\cite{he2015delving, hassan2018achieving, mstweet2018} 
% are paired with anthropomorphic descriptions of tasks, e.g. \citep{mstweet2018}:
% e.g. ``translation'' \citep{hassan2018achieving} and reading comprehension \citep{mstweet2018}, e.g.:
%
% \begin{displayquote}
% In a major milestone for \#MachineReading, Microsoft creates an \#AI that can read a document—and then answer questions about it—as well as a human \\
% -- @MSFTResearch
% \end{displayquote}
%
% The troubles with this Tweet are twofold: 
% (i) it uses the misleading term ``an AI'' 
% to describe a neural network, 
% (ii) it \emph{compares} human and ML performance without indicating that ML and human reading abilities \emph{are not comparable}: 
% the ML performance only holds on data drawn i.i.d. from the same distribution as the training data.
% By comparison, politicians worried about smashing ``the God particle'' might be comforted to learn that although ``God particle'' often comes up in pop-sci journalism, it's absent in formal scholarship.
% In contrast, a policymaker digging through published ML papers \emph{would} come across anthropomorphic language suggestive of human-like intelligence. 




==> sections/consequences.tex <==
% Folk wisdom might suggest not to intervene just as the field is heating up: 
% \emph{You can't argue with success!} 
% \emph{If it ain't broke, don't fix it!} 
% To counter these predictable objections, 
% we argue the following: 
% (i) the current culture is a \emph{consequence} 
% of ML's recent success, not its \emph{cause}; 
% and
% (ii) already, poor scholarship negatively impacts the research community and broader public. 

% \subsection{Misleading the public}

% \js{Probably want to move this somewhere else (and tone down substantially) but where? Potentially to discussion?}

% Consider the following example:
% the European parliament passed a report considering regulations to apply if ``robots become or are made self-aware'' \cite{eu2017}.
% %
% %\js{need a sentence explaining what is grossly mistaken and why}
% %
% At once it seems likely that the sudden interest in self-aware robots owes to reported developments in ML
% and yet no findings in ML to date suggest that we have made any progress towards conscious machines.
% But who could blame an outsider for mistaking 
% the character of machine learning's progress when authoritative peer-reviewed papers invoke terms like ``thought vector'' \citep{kiros2015skip} and ``consciousness prior'' \citep{bengio2017consciousness},
% when \emph{meaning} and \emph{co-occurrence} are casually interchanged, and when claims of human-level performance\cite{he2015delving, hassan2018achieving, mstweet2018} 
% are paired with exaggeratedly anthropomorphic descriptions of tasks, e.g. ``translation'' \citep{hassan2018achieving} and reading comprehension \citep{mstweet2018}, e.g.:
% %
% \begin{displayquote}
% In a major milestone for \#MachineReading, Microsoft creates an \#AI that can read a document—and then answer questions about it—as well as a human \\
% -- @MSFTResearch
% \end{displayquote}
% %
% The troubles with this Tweet are twofold: (i) it uses the misleading term ``an AI'' 
% to describe a neural network, (ii) it \emph{compares} human and ML performance without indicating that ML and human reading abilities \emph{are not comparable}: the ML performance only holds on data drawn i.i.d. from the same distribution as the training data.
% By comparison, politicians worried about smashing ``the God particle'' might be comforted to learn that although ``God particle'' often comes up in pop-sci journalism, it's absent in formal scholarship.
% In contrast, a policymaker digging through published ML papers \emph{would} come across anthropomorphic language suggestive of human-like intelligence. 


%\subsection{Confusing researchers}
%It's not only the layman comes to harm. 
%Researchers too are misled and confused due to lapses in scholarship.
%Let's revisit the case of deconvolution.

% More consequences of confusion among researchers are found by revisiting the case of ``internal covariate shift'' \cite{ioffe2015batch}.
% When introducing this new, vague term, the authors mischaracterize \emph{covariate shift} as simply a change in the distribution of the inputs. 
% In fact, \emph{covariate shift} refers to a specific restricted dataset shift 
% where although the input distribution $p(\mathbf{x})$ might change, 
% the labeling function $p(y|\mathbf{x})$ 
% does not \cite{gretton2009covariate}.
% This misunderstanding, coupled with the influence of \cite{ioffe2015batch}, 
% has created a situation in which the Google Scholar search engines, which relies heavily on markers of authority like citations \cite{beel2009google},
% lists batchnormalization as the first, most authoratitive reference in searches for ``covariate shift''.

==> sections/counterarguments.tex <==
%\js{Proposed refactor: Call these ``Countervailing Considerations'', state all of them (without providing counters), then counter once at the end by saying that these are all quite easy to do and shouldn't be interpreted as hard rules. I can make this refactor if you like it.}

%We anticipate a number of reasonable counterarguments 
%to our criticisms and suggestions. 
%To start, putting aside the issue
%to disrailing the public discourse,
%many readers might defend the status quo. 

We believe that greater rigor in both exposition, science, and theory are essential for both scientific progress and fostering a productive discourse with the broader public. 
Moreover, as practioners apply ML in critical domains such as health, law, and autonomous driving, a calibrated awareness of the abilities and limits of ML systems will enable us to deploy ML responsibly.
There are a number of countervailing considerations to the suggestions set forth above.

\subsection{Countervailing Considerations}
Several readers of earlier drafts of this paper noted
that \emph{stochastic gradient descent 
tends to converge faster than gradient descent}---in other words, perhaps a faster noisier process 
that ignores our guidelines for producing ``cleaner'' papers
results in a faster pace of research.
For example, the breakthrough paper 
on ImageNet  classification \citep{krizhevsky2012imagenet} 
proposes multiple techniques without ablation studies, 
several of which were subsequently determined 
to be unnecessary. 
However, at the time the results were so significant 
and the experiments so computationally expensive to run
that waiting for ablations to complete 
was perhaps not worth the cost to the community. 
%However, in many cases, addressing these issues
%only requires more careful writing 
%or several days of experiments.
% We believe that in these cases, papers can be improved without significant cost to the speed of progress and without restricting the diversity of technical research.

A related concern is that high standards might impede the publication of original ideas, which are more likely to be unusual and speculative. 
%Indeed, \emph{requiring} higher quality 
%by imposing strong restrictions on what can be published 
%carries the risk of slowing down progress. 
%The publishing climate in machine learning 
%is in many ways healthier than in other fields like economics 
In other fields such as economics,
high standards result in a publishing process 
that can take years for a single paper,
with lengthy revision cycles consuming resources 
that could be deployed towards new work.

Finally, perhaps there is value in \emph{specialization}:
the researchers generating new conceptual ideas 
or building new systems 
need not be the same ones who carefully collate and distill knowledge. 

We recognize the validity of these considerations, but contend that while the practices advocated here may take training to master, in many cases they are straightforward to implement, requiring only a few extra days of experiments and more careful writing. 
Moreover, we present these as strong heuristics rather than unbreakable rules---if an idea cannot be shared without violating these heuristics, we prefer the idea be shared and the heuristics set aside.
In short, we do not believe that the research community has achieved a Pareto optimal state on the growth-quality frontier. 




==> sections/recommendations.tex <==
Perhaps in an ideal world, 
all researchers would avoid all instances 
of the issues described above. 
However, we recognize that it takes training, skill, and hard work to be consistently precise in use of language and to adhere to rigorous scientific standards.
Moreover, even the best-trained and well-intentioned researchers will sometimes fall prey to some of the trends that we identified.
Moreover, we anticipate the counterargument that this is simply the price to be paid for growing the community, which we suspect most would agree is on balance desirable. 

\js{Other possible counterarguments:
\begin{itemize}
\item Specialization is good: shouldn't force good engineers and rigorous thinkers to be same people.
\item Forcing adherence to rigorous standards creates extra work for every paper that will slow down progress and isn't worth it. Retrospectives like the Melis et al. paper already correct errors efficiently.
\end{itemize}}

We do not believe that the research community has achieved a Pareto optimal state on the growth-quality frontier. 
To this end, we propose a set of concrete recommendations for debate.
These fall into three broad categories: 
improving academic standards, 
improving the review process, 
and improving incentives.

% or to develop a careful understanding of exactly why and when a method works well. 
% Even well-meaning researchers will fall prey to the trends that we identified. 
% Therefore, we focus our recommendations on actionable guidelines that can be conveyed to and followed by everyone.


\subsection{Improving Academic Standards} 
Three practices that are common in 
% the (in our opinion) 
the strongest empirical papers are 
\emph{error analysis},
\emph{ablation studies}, 
and \emph{robustness checks} 
(to e.g. choice of hyper-parameters, 
as well as ideally to choice of dataset). 
These practices can be adopted by everyone and we advocate their wide-spread use. For some papers that follow these practices we refer the reader to \citep{zhang2017tacred,liang2016neural}.  
% \js{double-check citations}

Broadly, we encourage authors to ask ``what worked?''~and ``why?'', rather than just ``how well?''. 
Except in extraordinary cases \citep{krizhevsky2012imagenet}, 
raw headline numbers provide limited value 
for scientific progress 
absent insight into what drives them. 
We stress that insight does not necessarily mean theory. 
Notable examples of empirical work aimed at insight 
include an exploration of loss surfaces 
of neural networks \citep{goodfellow2014qualitatively},
and a recent paper that demonstrated 
the ability of neural networks to fit 
randomly-assigned labels \citep{zhang2016understanding},
challenging the ability of established theory 
to explain the ability of neural networks to generalize to unseen data. \js{Maybe add Szegedy et al. \citep{szegedy2013intriguing} paper here?}

Finally, for reviewers, we recommend a heuristic to help create better incentives---\emph{ask, ``Would I have accepted this paper 
if the authors had done a worse job?''} \js{TODO: this heuristic confused some readers}
For instance, a paper describing a simple idea 
that leads to improved performance, 
together with two negative results,
should be judged more favorably 
than a paper that combines three ideas together 
(without ablation studies)
yielding the same improvement.

\subsection{Modifications to the Review Process} 

\js{This section was most controversial; I think we should remove most of it, and if we keep stuff acknowledge that many people have thought about this already and not clear there are easy answers.

Some thoughts on what we could say if we wanted to:
\begin{itemize}
\item Keep some version of desk rejection but phrase less negatively. For instance: ``It may help to include an \emph{author checklist} of easily actionable guidelines that authors should ensure they follow prior to submitting a paper. These might include for instance avoiding gaps between claims made in the abstract/intro and the rest of the paper. If a paper fails to follow the checklist, reviewers have the option of recommending rejection without a full review.''
\item Talk about recent efforts to improve things and how one might go even further (incentivizing good reviews).
\item Highlight some of the issues like the downward spiral.
\item Incorporate some suggestions from feedback e-mails?
\end{itemize}}

Even before the rapid growth of ML as a field, 
the conference review process was under stress; it is now approaching a breaking point. 
There are simply too many papers submitted 
relative to the number of experts 
qualified to review them. 


To address these issues, our first recommendation is to \emph{purge weak reviewers}. 
It is tempting to include everyone who is willing and even plausibly able as a reviewer, 
often by inviting anyone who has published 
at least $X$ papers in the past few years. 
However, this has the insidious effect 
that compromised standards 
lead to a downward spiral---once a subpar paper is accepted, 
the authors enter the pool of reviewers.
As a first-pass approach, one could only invite authors to review whose average score in clarity and technical merit is above a sufficiently high threshold (demonstrating by example that they can recognize good papers), 
and ask area chairs to evaluate reviewers 
at the end of the reviewing cycle 
(dis-inviting reviewers with 
consistently low evaluations).  %\js{TODO: motivate this approach more?}
% \js{Note that NIPS appears to perhaps be implementing that this year?}

One obvious problem with this approach 
is that it further thins an already-stretched reviewer pool. 
To compensate for this, 
we recommend instituting \emph{desk rejections}. 
Papers with clear unacceptable defects 
can be rejected with the review of only a single expert reviewer (together with the area chair). 
Such problems could include: 
excessive typos or obvious lack or proofreading; 
gap between claims made in the abstract/intro 
and the rest of the paper; 
or serious flaws in the theory or experimental results. 
Even if a paper is otherwise strong, 
these are clear flaws 
that should be fixed before final publication, 
and it's fine to ask authors 
to resubmit in the next cycle. 

An important aspect of our proposal 
is that issues leading to desk rejection 
are clearly articulable 
and objectively addressable; 
this means that all authors should be capable 
of eventually bringing a paper into a state 
that is ready for full peer review.

\subsection{Setting Better Incentives for Authors} 

\js{We already talk about incentives above; should merge it with this part}

We focus here on positively incentivizing work 
that pushes back against the negative trends 
that we identified. 
We feel the current system under-values \emph{retrospective surveys} and 
%\emph{high-quality speculation} and 
discuss changes to address this. %\js{don't currently discuss the latter}
Current literature moves fast at the expense of accepting flawed works for conference publication. One remedy could be to emphasize  authoritative retrospective surveys 
that strip out exaggerated claims and extraneous material, change anthropomorphic names to sober alternatives, standardize notation, etc. 
We recommend creating proper tracks for these authoritative syntheses of recent research. 
While these surveys would be published and presented at conferences, we advocate subjecting them to journal-type reviewing, including a revision cycle and conditional acceptance, in order to ensure consistently high quality.

\js{should probably cite Distill (although it is slightly different)}

% \js{possibly expand further?}

% \js{Somewhat inclined to delete this point since it's much weaker/tangential than the others in this section.} Perhaps more controversially, 
% we propose that the prevalence of speculation i
% in technical ML papers may be due in part
% to the paucity of venues 
% for high-quality peer-reviewed work 
% of a speculative nature. 
% % Here we distinguish low-quality speculation (which is rarely well-supported and often presented as fact) from high-quality speculation (which is explicitly marked as such and often has substantial but not conclusive supporting arguments). 
% Providing a peer-reviewed venue for speculation, opinion, and discussions of long-term trajectory of research and its impacts, 
% if done correctly, 
% could help to clean up the technical conferences while providing a venue for the community to adopt a more rigorous forward-looking stance. 
% % ZL removing the throat clearing
% % Such an outcome would be sufficiently beneficial that we advocate attempting to achieve it despite its arguably quixotic nature.

% \section{Conclusions}
% % \zl{address the predictable counter -- isn't this just the cost for having a big community? - perhaps bring that up before recommendations.}
% In this essay, 
% we expand upon these ills and their consequences. 
% We then explain some possible causes of the present crisis in scholarship, 
% including the dilution of the reviewer pool, the poorly aligned incentives 
% of scholarship and press coverage, 
% and the relatively rapid expansion 
% of the research community 
% in comparison to the ranks 
% of qualified mentors.
% Finally, we present some concrete recommendations, such as instituting desk rejects, culling the reviewer pool, designing  rigorous reviewing guidelines, and creating  greater incentives (such as first-tier ICLR/ICML/NIPS proceedings) for clear surveys of recent advances that meet higher bars 
% for pedagogy and sobriety 
% than the primary literature. 



